Measurement of the top quark pair production charge asymmetry in proton-proton collisions at 7 TeV using the ATLAS detector

This letter presents a measurement of the top quark pair (tt) production charge asymmetry Ac using 4.7 fb-1 of proton-proton collisions at a centre-of-mass energy of 7 TeV collected by the ATLAS detector at the LHC. A tt-enriched sample of events with a single lepton (electron or muon), missing transverse momentum and at least four high transverse momentum jets, of which at least one is tagged as coming from a b-quark, is selected. A likelihood fit is used to reconstruct the tt event kinematics. A Bayesian unfolding procedure is employed to estimate Ac at the parton-level. The measured value of the tt production charge asymmetry is 0.006 +/- 0.010, where the uncertainty includes both the statistical and the systematic components. Differential Ac measurements as a function of the invariant mass, the rapidity and the transverse momentum of the tt-system are also presented. In addition, Ac is measured for a subset of events with large tt velocity, where physics beyond the Standard Model could contribute. All measurements are consistent with the Standard Model predictions.

==> Interpretation.tex <==
\begin{figure}[htp]
\begin{center}
\includegraphics[width=0.45\textwidth]{AFB-ATLAS-2013.pdf}
\includegraphics[width=0.45\textwidth]{AFB-ATLAS450vs600-2013.pdf}
%\includegraphics[width=0.9\columnwidth,scale=0.2]{AFB-ATLAS-2013.pdf}
%\includegraphics[width=0.9\columnwidth,scale=0.2]{AFB-ATLAS450vs600-2013.pdf}
\caption{Measured forward--backward asymmetries $A_{\rm{FB}}$ at Tevatron and charge asymmetries \Ac\ at LHC, 
compared with the SM predictions (black box) as well as predictions incorporating various potential new physics contributions (as described in the figure)~\cite{AguilarSaavedra:2011hz,AguilarSaavedra:2011ug}.
In both plots, where present, the horizontal bands and lines correspond to the ATLAS (light green) and CMS (dark green) measurements, while the vertical ones correspond to
the CDF (orange) and D0 (yellow) measurements.
The inclusive \Ac\ measurements are reported in the left plot. In the right plot a comparison is reported between the $A_{\rm{FB}}$ measurement by CDF for $\mttbar > 450$ \GeV\ and the 
\Ac\ measurement for $\mttbar > 600$ \GeV.}
\label{fig:AvsA}
\end{center}
\end{figure}


==> table_systematics.tex <==
\begin{table*}[tbp]
\begin{center}
{\footnotesize
\begin{tabular}{|l |c |c|}
\hline
Source of systematic uncertainty  & \multicolumn{2}{|c|}{$\delta{\Ac}$} \\
\hline
  & Inclusive & $\mttbar >600$ \GeV \\
\hline
Lepton reconstruction/identification	& $<0.001$ & 0.001 \\
Lepton energy scale and resolution	& 0.003 & 0.003\\
Jet energy scale and resolution		& 0.003 & 0.003\\
Missing transverse momentum and pile--up modelling & 0.002 & 0.002\\
Multi--jets background normalisation	& $<0.001$ & 0.001\\
$b$--tagging/mis--tag efficiency	& $<0.001$ & 0.001\\
Signal modelling			& $<0.001$ & $<0.001$\\
Parton shower/hadronisation		& $<0.001$  & $<0.001$\\
Monte Carlo statistics			& 0.002  & $<0.001$\\
PDF					& 0.001  & $<0.001$\\
$W$+jets normalisation and shape        & 0.002  & $<0.001$\\
\hline
Statistical uncertainty			& 0.010 & 0.021\\
\hline 
\end{tabular}
}
\caption{\label{Table_Systematics}Systematic uncertainties for the inclusive asymmetry, \Ac\ (central column), and the asymmetry for  $\mttbar > 600$ \GeV(right column).
For variations resulting in asymmetric uncertainties, the average absolute deviation from
the nominal value is reported. The values reported for each systematic uncertainty are the variation of the mean of posteriors computed considering 1$\sigma$ variations.}
\end{center}
\end{table*}

